Train Scheduling with Hybrid Answer Set Programming

We present a solution to real-world train scheduling problems, involving routing, scheduling, and optimization, based on Answer Set Programming (ASP). To this end, we pursue a hybrid approach that extends ASP with difference constraints to account for a fine-grained timing. More precisely, we exemplarily show how the hybrid ASP system clingo[DL] can be used to tackle demanding planning-and-scheduling problems. In particular, we investigate how to boost performance by combining distinct ASP solving techniques, such as approximations and heuristics, with preprocessing and encoding techniques for tackling large-scale, real-world train scheduling instances. Under consideration in Theory and Practice of Logic Programming (TPLP)

==> acknowledgments.tex <==
\noindent
\emph{Acknowledgments}
%
This work was partially funded by DFG grants SCHA 550/9 and~11.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> data/aggregates.tex <==
\binary{}-\standard             & 4767 & 175 &  4136 & 165 & 2578 & 165 &  3215 & 175 &  \textbf{684} & 165 \\
\binary{}-\threads{2}           &  933 & 181 &  *575 & 184 &  937 & 173 &   909 & 175 &  \textbf{574} & \textbf{165}\\
\binary{}-\threads{2}-\bb       & 5050 & 166 &  4723 & 175 & 2481 & 165 &  1916 & 177 &  \textbf{600} & 165\\
\binary{}-\threads{2}-\usc      & *877 & 165 &   581 & 184 & *881 & 165 &  *881 & 175 &  \textbf{574} & 173\\
\linear{}-\standard             & \na  & \na & 23343 &  33 & 6380 &  33 &   \na & \na &  \textbf{705} &  33\\
\linear{}-\threads{2}           & 1118 &  33 &   694 &  33 & 1264 &  33 &   926 &  33 &  \textbf{611} &  33\\
\linear{}-\threads{2}-\bb       & \na  & \na & 16495 &  33 & 4561 &  33 & 11667 &  33 &  \textbf{605} &  33\\
\linear{}-\threads{2}-\usc      & 4047 &  33 &  \textbf{2351} &  33 & \na  & \na &   \na & \na &  \na &  \na

==> data/instances.tex <==
1 & 4   &  159  &   159 &   2 &     0 &      0 &   2 &      0 &     0 \\
2 & 58  & 1839  &  1816 &   5 &     0 &      0 &   5 &      0 &     0 \\
3 & 143 & 2117  &  2090 &   8 &     0 &      0 &   9 &      0 &     0 \\
4 & 148 & 2371  &  2352 &  12 &     0 &      0 &  13 &      0 &     0 \\
5 & 149 & 2376  &  2356 &  19 &     8 &    165 &  42 &     21 &    33 \\
6 & 365 & 3128  &  3109 & 149 &     0 &      0 & 144 &      0 &     0 \\
7 & 467 & 3128  &  3109 & 252 &     0 &      0 & 251 &      0 &     0 \\
8 & 133 & 3228  &  3314 & 127 &     0 &      0 & 139 &      0 &     0 \\
9 & 287 & 34488 & 34827 & \na &   \na &    \na & \na &    \na &   \na \\
